The Case for Strong Scaling in Deep Learning: Training Large 3D CNNs with Hybrid Parallelism

We present scalable hybrid-parallel algorithms for training large-scale 3D convolutional neural networks. Deep learning-based emerging scientific workflows often require model training with large, high-dimensional samples, which can make training much more costly and even infeasible due to excessive memory usage. We solve these challenges by extensively applying hybrid parallelism throughout the end-to-end training pipeline, including both computations and I/O. Our hybrid-parallel algorithm extends the standard data parallelism with spatial parallelism, which partitions a single sample in the spatial domain, realizing strong scaling beyond the mini-batch dimension with a larger aggregated memory capacity. We evaluate our proposed training algorithms with two challenging 3D CNNs, CosmoFlow and 3D U-Net. Our comprehensive performance studies show that good weak and strong scaling can be achieved for both networks using up 2K GPUs. More importantly, we enable training of CosmoFlow with much larger samples than previously possible, realizing an order-of-magnitude improvement in prediction accuracy.

==> performance.tex <==
\makeatletter

\newcommand{\perfoutdated}{\textcolor{red!80!black}{$\blacktriangle$}}

% From the CosmoFlow SC18 paper
\@namedef{dim128-forward-flops}{18.5 GFlops}
\@namedef{dim128-num-params}{9.44 M}

% From the ResNet paper
\@namedef{resnet152-forward-flops}{1.13 GFlops}

% scripts/201905_4parE/out_summary.csv
\@namedef{dim128-training-test-mse}{0.0435}
\@namedef{dim256-training-test-mse}{0.0169}
\@namedef{dim512-training-test-mse}{0.00727}
\@namedef{dim512bn-training-test-mse}{0.00445}
\@namedef{dim256-eighth-training-test-mse}{0.156} % 0.15554, lbann/distconv_dim256_eighth/20190513_182331_0.0005_N32_BS128_Nx1x1x1

% scripts/201905_4parE/plot.r time
\@namedef{dim128-training-time}{5.99 h}
\@namedef{dim256-training-time}{2.52 h}
\@namedef{dim512-training-time}{2.15 h}
\@namedef{dim512bn-training-time}{2.08 h}

% dim128-training-time / dim512bn-training-time
% Here I don't use dim512bn because it uses double number of GPUs and incurs additional amount of computation (the BN layers),
% so the comparison might be unclear/unfair.
\@namedef{training-speedup-dim128-dim512}{2.79x}

% 3550 GFlops/sample * 10012 samples * 0.8 / 56.872150000000005s
% The epoch time comes from 20191012_102317_512_0.001_N128_BS64_Nx8x1x1
\@namedef{dim512bn-training-eff-flops}{500 FP32 TFlop/s}
\@namedef{dim512bn-training-num-gpus}{512} % 128 nodes

% From scripts/weak_scale/plot.r
\@namedef{weak-scale-speedup-dim128-n1-to-n128}{65.4x}
\@namedef{weak-scale-ratio-dim512bn-n128-nx8x1x1-to-nx16x1x1}{1.35x}
\@namedef{weak-scale-sps-dim512bn-n64-nx8x1x1}{88.9 samples/s}
\@namedef{weak-scale-sps-dim512bn-n128-nx16x1x1}{121.3 samples/s}
\@namedef{weak-scale-sps-dim512bn-n128-nx8x1x1}{163.5 samples/s}
\@namedef{weak-scale-speedup-dim512bn-nx8x1x1-n2-to-n128}{49.9x}
\@namedef{weak-scale-speedup-dim512bn-nx16x1x1-n4-to-n128}{21.2x}
\@namedef{weak-scale-speedup-dim512bn-n64-nx8x1x1-to-n128-nx16x1x1}{1.36x} % weak-scale-sps-dim512bn-n128-nx16x1x1 / weak-scale-sps-dim512bn-n64-nx8x1x1

\@namedef{weak-scale-speedup-dim512bn-nx8x1x1-n2-to-n512}{147.31x}
\@namedef{weak-scale-speedup-dim512bn-nx16x1x1-n4-to-n512}{71.32x}
\@namedef{weak-scale-speedup-dim512bn-nx32x1x1-n8-to-n512}{37.2x}

\@namedef{weak-scale-speedup-unet-dim256-bn-n8-to-n256}{28.4x}

% 3550 GFlops/sample * weak-scale-sps-dim512bn-n128-nx8x1x1
\@namedef{weak-scale-dim512bn-nx8x1x1-flops}{580 FP32 TFlop/s}
% Flop/s / 56 [GFlop/s/node] * 128 nodes
\@namedef{weak-scale-dim512bn-nx2x2x1-flops-eff}{13.3\%}

% From scripts/strong_scale_breakdown/plot.r
\@namedef{strong-scale-cosmoflow-speedup-N4-n8-to-n32}{2.15x}
\@namedef{strong-scale-cosmoflow-speedup-N4-n8-to-n16}{1.66x}
\@namedef{strong-scale-cosmoflow-speedup-N16-n32-to-n128}{1.98x}
\@namedef{strong-scale-cosmoflow-speedup-N16-n32-to-n256}{2.12x}
\@namedef{strong-scale-cosmoflow-speedup-N64-n128-to-n512}{1.77x}

\@namedef{strong-scale-unet-speedup-N16-n64-to-n128}{1.42x}

% From scripts/performance_model/plot_conv.r
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-layer}{conv1}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-time}{69.5}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-tflops}{13.0} %1.62
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-eff}{10.3}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-time}{136.6}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-tflops}{23.6} %2.95
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-eff}{18.8}
\@namedef{performance-model-conv-cosmoflow-depth8-conv1-forward-flop-ratio}{20.8\%}
\@namedef{performance-model-conv-cosmoflow-depth8-conv1-backward-data-flop-ratio}{0.0\%}
\@namedef{performance-model-conv-cosmoflow-depth8-conv1-backward-filter-flop-ratio}{6.8\%}
\@namedef{performance-model-conv-cosmoflow-depth8-time-total}{136 ms}
\@namedef{performance-model-conv-cosmoflow-depth8-flop-ratio-total}{18.8\%}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-layer}{conv1}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-time}{15.2}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-tflops}{53.4} %1.67
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-eff}{10.7}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-time}{40.3}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-tflops}{109.1} %3.41
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-eff}{21.7}
\@namedef{performance-model-conv-cosmoflow-depth32-conv1-forward-flop-ratio}{22.0\%}
\@namedef{performance-model-conv-cosmoflow-depth32-conv1-backward-data-flop-ratio}{0.0\%}
\@namedef{performance-model-conv-cosmoflow-depth32-conv1-backward-filter-flop-ratio}{7.0\%}
\@namedef{performance-model-conv-cosmoflow-depth32-time-total}{40 ms}
\@namedef{performance-model-conv-cosmoflow-depth32-flop-ratio-total}{21.7\%}
\@namedef{performance-model-conv-unet-depth16-dominant-layer}{7-1}
\@namedef{performance-model-conv-unet-depth16-dominant-time}{149.0}
\@namedef{performance-model-conv-unet-depth16-dominant-tflops}{12.51}
\@namedef{performance-model-conv-unet-depth16-dominant-eff}{79.7}
\@namedef{performance-model-conv-unet-depth16-dominant-all-time}{579.5}
\@namedef{performance-model-conv-unet-depth16-dominant-all-tflops}{11.05}
\@namedef{performance-model-conv-unet-depth16-dominant-all-eff}{70.4}
\@namedef{performance-model-conv-unet-depth16-conv7-1-forward-flop-ratio}{93.1\%}
\@namedef{performance-model-conv-unet-depth16-conv7-1-backward-data-flop-ratio}{69.6\%}
\@namedef{performance-model-conv-unet-depth16-conv7-1-backward-filter-flop-ratio}{79.8\%}
\@namedef{performance-model-conv-unet-depth16-time-total}{579 ms}
\@namedef{performance-model-conv-unet-depth16-flop-ratio-total}{70.4\%}
\@namedef{performance-model-conv-unet-depth32-dominant-layer}{conv7}
\@namedef{performance-model-conv-unet-depth32-dominant-time}{64.4}
\@namedef{performance-model-conv-unet-depth32-dominant-tflops}{12.41}
\@namedef{performance-model-conv-unet-depth32-dominant-eff}{79.0}
\@namedef{performance-model-conv-unet-depth32-dominant-all-time}{328.3}
\@namedef{performance-model-conv-unet-depth32-dominant-all-tflops}{10.83}
\@namedef{performance-model-conv-unet-depth32-dominant-all-eff}{69.0}
\@namedef{performance-model-conv-unet-depth32-conv7-1-forward-flop-ratio}{88.2\%}
\@namedef{performance-model-conv-unet-depth32-conv7-1-backward-data-flop-ratio}{69.5\%}
\@namedef{performance-model-conv-unet-depth32-conv7-1-backward-filter-flop-ratio}{81.7\%}
\@namedef{performance-model-conv-unet-depth32-time-total}{328 ms}
\@namedef{performance-model-conv-unet-depth32-flop-ratio-total}{69.0\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-layer}{conv7}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-time}{238.0}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-tflops}{125.3} %7.83
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-eff}{49.9}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-time}{734.3}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-tflops}{139.5} %8.72
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-eff}{55.5}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-conv7-1-forward-flop-ratio}{45.4\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-conv7-1-backward-data-flop-ratio}{39.0\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-conv7-1-backward-filter-flop-ratio}{80.0\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-time-total}{734 ms}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-flop-ratio-total}{55.5\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-layer}{conv7}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-time}{99.2}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-tflops}{257.6} %8.05
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-eff}{51.3}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-time}{388.0}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-tflops}{293.4} %9.17
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-eff}{58.4}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-conv7-1-forward-flop-ratio}{45.8\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-conv7-1-backward-data-flop-ratio}{40.9\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-conv7-1-backward-filter-flop-ratio}{82.0\%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-time-total}{387 ms}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-flop-ratio-total}{58.4\%}

% Computed manually % TODO: automate the computation
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-time-actual}{142.9}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-time-actual}{48.8}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-time-actual}{693.5}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-time-actual}{386.6}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-tflops-actual}{22.6} %2.82
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-tflops-actual-relative-to-cudnn}{95.6}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-tflops-actual}{89.9} %2.81
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-tflops-actual-relative-to-cudnn}{82.4}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-tflops-actual}{147.7} %9.23
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-tflops-actual-relative-to-cudnn}{105.8}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-tflops-actual}{294.4} %9.20
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-tflops-actual-relative-to-cudnn}{100.3}
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-all-eff-actual}{18.0}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-all-eff-actual}{17.9}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-all-eff-actual}{58.8}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-all-eff-actual}{58.6}

\@namedef{performance-model-conv-cosmoflow-depth8-dominant-time-actual}{73.9}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-time-actual}{23.5}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-time-actual}{237.0}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-time-actual}{121.7}

\@namedef{performance-model-conv-cosmoflow-depth8-dominant-tflops-actual}{12.2} %1.52
\@namedef{performance-model-conv-cosmoflow-depth8-dominant-tflops-actual-relative-to-cudnn}{93.8}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-tflops-actual}{34.6} % 1.08
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-tflops-actual-relative-to-cudnn}{64.7}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-tflops-actual}{125.9} %7.87
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-tflops-actual-relative-to-cudnn}{100.5}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-tflops-actual}{210.2} %6.57
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-tflops-actual-relative-to-cudnn}{81.6}

\@namedef{performance-model-conv-cosmoflow-depth8-dominant-eff-actual}{9.7}
\@namedef{performance-model-conv-cosmoflow-depth32-dominant-eff-actual}{6.9}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-dominant-eff-actual}{50.1}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-dominant-eff-actual}{41.8}

\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-flop-ratio-total-actual}{58.8 \%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-flop-ratio-total-actual}{58.6 \%}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth16-time-total-actual}{693.5 ms}
\@namedef{performance-model-conv-unet-conv-ws0.001-depth32-time-total-actual}{386.6 ms}

\@namedef{performance-model-conv-cosmoflow-depth8-flop-ratio-total-actual}{18.0 \%}
\@namedef{performance-model-conv-cosmoflow-depth32-flop-ratio-total-actual}{17.9 \%}
\@namedef{performance-model-conv-cosmoflow-depth32-time-total-actual}{48.8 ms}

\@namedef{n411}{$4$-way}
\@namedef{n221}{$2 \times 2$-way}
\@namedef{n811}{$8$-way}
\@namedef{n1611}{$16$-way}

\@namedef{dim128}{$128^3$}
\@namedef{dim256}{$256^3$}
\@namedef{dim512}{$512^3$}

\makeatother


==> tables/accuracy_comparison.tex <==
% Run 201905_4parE_residuals to get the table.

\ifthenelse{\isundefined{\accuracycomparisonforslides}}{
  \newcommand{\sabf}[1]{#1}
}{
  \newcommand{\sabf}[1]{\alertbf{#1}}
}

\begin{tabular}{c|c c c c}
  \toprule
  & $\Omega_m$ & $\sigma_8$ & $n_s$ & $H_0$ \\
  % \midrule
  % Previous work \cite{Mathuriya:2018:CUD:3291656.3291743} & 0.0022 & 0.0094 & 0.0096 & N/A \\
  \midrule
  \perf{dim128} & 0.0380 & 0.0380 & 0.0394 & 0.0751 \\
  \perf{dim256} & 0.0234 & 0.0241 & 0.0256 & 0.0468 \\
  \perf{dim512} & 0.0158 & 0.0167 & 0.0188 & 0.0285 \\
  \sabf{\perf{dim512}, BN} & \sabf{0.0102} & \sabf{0.0126} & \sabf{0.0142} & \sabf{0.0241} \\
  \bottomrule
\end{tabular}


==> tables/comparison_strategy.tex <==
\begin{tabular}{c|c c c}
  \toprule
  & \textbf{Data} & \textbf{Model} & \textbf{Hybrid} \\
  \midrule
  \textbf{What to parallelize} & Samples & Layers & Samples \& layers \\
  \textbf{Available parallelism} & $O(N)$ & $O(W^n)$ & \textcolor{green!50!black}{$O(N W^n)$} \\
  \textbf{GPU memory pressure} & \xmark & \cmark & \cmark \\
  \textbf{Influence on accuracy} & \xmark & \cmarkplus & \cmark \\
  \textbf{Weak scaling} & \cmark & N/A & \cmark \\
  \textbf{Strong scaling} & \cmarkplus & \cmark & \cmarkplus \\
  \bottomrule
\end{tabular}


==> tables/flops.tex <==
% From scripts/distconv/distconv_1gpu/out_num_flops_v100.tex
\begin{tabular}{c|c c c}
  \toprule
  Name & Forward & Backward data & Backward filter \\
       & [GFlops] & [GFlops] & [GFlops] \\
  \midrule
  conv1 & 1.81 & 1.81 & 1.81 \\
  conv2 & 7.25 & 7.25 & 7.25 \\
  conv3 & 3.62 & 3.62 & 3.62 \\
  conv4 & 0.03 & 0.03 & 0.03 \\
  conv5 & 0.91 & 0.91 & 0.91 \\
  conv6,7 & 1.81 & 1.81 & 1.81 \\
  \bottomrule
\end{tabular}


==> tables/network_comparison.tex <==
\begin{tabular}{c c c c|c}
  \toprule
  Network & \# nodes & $N$ & $\eta^{(0)}$ & Test loss \\
  \midrule
  Baseline & 8   & \num{512}  & $1 \times 10^{-4}$ & 0.0051 \\
  Baseline & 32  & \num{2048} & $2 \times 10^{-4}$ & 0.0077 \\
  Baseline & 128 & \num{8192} & $5 \times 10^{-4}$ & 0.0184 \\
  \midrule
  CO       & 64  & \num{2048} & $1.5 \times 10^{-4}$ & 0.0073 \\
  C3       & 64  & \num{2048} & $3   \times 10^{-4}$ & 0.0077 \\
  C3P3     & 32  & \num{1024} & $1   \times 10^{-4}$ & 0.0057 \\
  C3P3P2   & 32  & \num{1024} & $2   \times 10^{-4}$ & 0.0041 \\
  \bottomrule
\end{tabular}

% \begin{tabular}{c c c c|c c}
%   \toprule
%   \multirow{2}{*}{Network} & Number of & \multirow{2}{*}{$N$} & \multirow{2}{*}{$\eta^{(0)}$} & \multicolumn{2}{c}{Minimum loss} \\
%   & nodes & & & Training & Test \\
%   \midrule
%   Original & 8   &   512 & 0.0001 & 0.0041 & 0.0051 \\
%   Original & 32  & 2,048 & 0.0002 & 0.0110 & 0.0077 \\
%   Original & 128 & 8,192 & 0.0005 & 0.0241 & 0.0184 \\
%   \midrule
%   CO       & 64  & 2,048 & 0.00015 & 0.0093 & 0.0073 \\
%   C3       & 64  & 2,048 & 0.0003  & 0.0106 & 0.0077 \\
%   C3P3     & 32  & 1,024 & 0.0001  & 0.0076 & 0.0057 \\
%   C3P3P2   & 32  & 1,024 & 0.0002  & 0.0062 & 0.0041 \\
%   \bottomrule
% \end{tabular}


==> tables/network_summary.tex <==
\begin{tabular}{c|c c c}
  \toprule
  \textbf{Input width ($W$)} & \textbf{128} & \textbf{256} & \textbf{512} \\
  \textbf{\# of input channels ($C$)} & \textbf{4} & \textbf{4} & \textbf{4} \\
  \midrule
  \textbf{\# of samples} & 65,728 & 8,216 & 1,027 \\
  \textbf{Dataset size [TiB]} & 1.00 & 1.00 & 1.00 \\
  \midrule
  \textbf{\# of conv. ops. [GFlops/sample]} & 55.55 & 443.8 & 3550 \\ % Use c3p3p2_flops.py to compute this
  \textbf{(Forward)} & 18.52 & 147.9 & 1183 \\
  \textbf{Memory [GiB/sample]} & 0.824 & 6.59 & \textcolor{red!75!black}{\textbf{52.7}} \\ % Use compute_tensor_memory.py to compute this
  \textbf{\# of parameters [$10^6$]} & 9.44 & 9.44 & 9.44 \\ % Use compute_num_weights.py to compute this
  \bottomrule
\end{tabular}

